CloudPowerCap: Integrating Power Budget and Resource Management across a Virtualized Server Cluster

In many datacenters, server racks are highly underutilized. Rack slots are left empty to keep the sum of the server nameplate maximum power below the power provisioned to the rack. And the servers that are placed in the rack cannot make full use of available rack power. The root cause of this rack underutilization is that the server nameplate power is often much higher than can be reached in practice. To address rack underutilization, server vendors are shipping support for per-host power caps, which provide a server-enforced limit on the amount of power that the server can draw. Using this feature, datacenter operators can set power caps on the hosts in the rack to ensure that the sum of those caps does not exceed the rack's provisioned power. While this approach improves rack utilization, it burdens the operator with managing the rack power budget across the hosts and does not lend itself to flexible allocation of power to handle workload usage spikes or to respond to changes in the amount of powered-on server capacity in the rack. In this paper we present CloudPowerCap, a practical and scalable solution for power budget management in a virtualized environment. CloudPowerCap manages the power budget for a cluster of virtualized servers, dynamically adjusting the per-host power caps for hosts in the cluster. We show how CloudPowerCap can provide better use of power than per-host static settings, while respecting virtual machine resource entitlements and constraints.

==> acks.tex <==
\section*{Acknowledgments}

We are thankful to all the engineers who worked on the DRS and Storage DRS
products which our work is built on. We would like to thank Anne Holler,
Irfan Ahmad, Shankari Kalyanaraman, Limin Wang, Jyothir Ramanan and 
Aashish Parikh for various discussions.
We are also very grateful to Bala Kaushik, Ajit Mayya and Thuan Pham for 
motivating us to work on these problems.
%\vfill\eject


==> cases_fig.tex <==
\begin{figure}[htpb]
    \centering
  \begin{minipage}{5in}\subfloat[{\small Enable VMs movement}]{
    \centering
    \begin{tikzpicture}[y=.25cm, x=.25cm,font=\sffamily, scale=0.7]
        % host 1
        \draw[fill=blue!5, rounded corners = 2pt, drop shadow, very
        thick, draw=gray] (0, 0)
        rectangle (8,10);
        \draw (4, 11) node{\scriptsize \textbf{Host A}};
        % host 2
        \draw[fill=blue!5, rounded corners = 2pt, drop shadow, very
        thick, draw=gray] (10, 0)
        rectangle (18,10);
        \draw (14, 11) node{\scriptsize \textbf{Host B}};
        % vm for host 1
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (0, 0)
        rectangle (8,2);
        \draw (4, 1) node{\scriptsize \color{White}{\textbf{VM 1}}};        
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (0, 2)
        rectangle (8,6);
        \draw (4, 4) node{\scriptsize \color{White}{\textbf{VM 2}}};        
        % vm for host 2
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (10, 0)
        rectangle (18,5);
        \draw (14, 2.5) node{\scriptsize \color{White}{\textbf{VM 3}}};        
        % capped capacity
        \path [draw, thick, color=red!80, dashed] (0, 8) -- (8, 8);
        \draw (4, 8.7) node{\scriptsize \color{Black!60}{\textbf{CC}}};
        \path [draw, thick, color=red!80, dashed] (10, 8) -- (18, 8);
        \draw (14, 8.7) node{\scriptsize \color{Black!60}{\textbf{CC}}};
      \end{tikzpicture}\quad\quad\quad
    \centering
    \begin{tikzpicture}[y=.25cm, x=.25cm,font=\sffamily, scale=0.7]
        % host 1
        \draw[fill=blue!5, rounded corners = 2pt, drop shadow, very
        thick, draw=gray] (0, 0)
        rectangle (8,10);
        \draw (4, 11) node{\scriptsize \textbf{Host A}};
        % host 2
        \draw[fill=blue!5, rounded corners = 2pt, drop shadow, very
        thick, draw=gray] (10, 0)
        rectangle (18,10);
        \draw (14, 11) node{\scriptsize \textbf{Host B}};
        % vm for host 1
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (0, 0)
        rectangle (8,2);
        \draw (4, 1) node{\scriptsize \color{White}{\textbf{VM 1}}};        
        % vm for host 2
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (10, 0)
        rectangle (18,5);
        \draw (14, 2.5) node{\scriptsize \color{White}{\textbf{VM 3}}};        
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (10, 5)
        rectangle (18,9);
        \draw (14, 7) node{\scriptsize \color{White}{\textbf{VM 2}}};        
        % capped capacity
        \path [draw, thick, color=red!80, dashed] (0, 6) -- (8, 6);
%        \path [draw, thick, color=red!80, dashed] (0, 8) -- (8, 8);
        \draw (4, 6.7) node{\scriptsize \color{Black!60}{\textbf{CC}}};
      \end{tikzpicture}
    \label{fig:vmmove}
  } \end{minipage}\\
    \centering
  \subfloat[{\small Improve robustness}]{
    \centering
    \begin{tikzpicture}[y=.25cm, x=.25cm,font=\sffamily, scale=0.7]
        % host 1
        \draw[fill=blue!5, rounded corners = 2pt, drop shadow, very
        thick, draw=gray] (0, 0)
        rectangle (8,10);
        \draw (4, 11) node{\scriptsize \textbf{Host A}};
        % host 2
        \draw[fill=blue!5, rounded corners = 2pt, drop shadow, very
        thick, draw=gray] (10, 0)
        rectangle (18,10);
        \draw (14, 11) node{\scriptsize \textbf{Host B}};
        % vm for host 1
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (0, 0)
        rectangle (8,4);
        \draw (4, 2) node{\scriptsize \color{White}{\textbf{VM 2}}};        
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (0, 4)
        rectangle (8,6);
        \draw (4, 5) node{\scriptsize \color{White}{\textbf{VM 1}}};        
        % vm for host 2
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (10, 0)
        rectangle (18,5);
        \draw (14, 2.5) node{\scriptsize \color{White}{\textbf{VM 3}}};        
        % capped capacity
        \path [draw, thick, color=red!80, dashed] (0, 8) -- (8, 8);
        \draw (4, 8.7) node{\scriptsize \color{Black!60}{\textbf{CC}}};
        \path [draw, thick, color=red!80, dashed] (10, 8) -- (18, 8);
        \draw (14, 8.7) node{\scriptsize \color{Black!60}{\textbf{CC}}};
      \end{tikzpicture}\quad\quad\quad
    \centering
    \begin{tikzpicture}[y=.25cm, x=.25cm,font=\sffamily, scale=0.7]
        % host 1
        \draw[fill=blue!5, rounded corners = 2pt, drop shadow, very
        thick, draw=gray] (0, 0)
        rectangle (8,10);
        \draw (4, 11) node{\scriptsize \textbf{Host A}};
        % host 2
        \draw[fill=blue!5, rounded corners = 2pt, drop shadow, very
        thick, draw=gray] (10, 0)
        rectangle (18,10);
        \draw (14, 11) node{\scriptsize \textbf{Host B}};
        % vm for host 1
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (0, 0)
        rectangle (8,4);
        \draw (4, 2) node{\scriptsize \color{White}{\textbf{VM 2}}};        
        % vm for host 2
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (10, 0)
        rectangle (18,5);
        \draw (14, 2.5) node{\scriptsize \color{White}{\textbf{VM 3}}};        
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (10, 5)
        rectangle (18,7);
        \draw (14, 6) node{\scriptsize \color{White}{\textbf{VM 1}}};        
        % capped capacity
        \path [draw, thick, color=red!80, dashed] (0, 6) -- (8, 6);
        \draw (4, 6.7) node{\scriptsize \color{Black!60}{\textbf{CC}}};
      \end{tikzpicture}
    \label{fig:vmrobust}
  } \\
  \subfloat[{\small Reduces {overhead~of~entitlement~balancing}}]{
    \centering
    \begin{tikzpicture}[y=.25cm, x=.25cm,font=\sffamily, scale=0.7]
        % host 1
        \draw[fill=blue!5, rounded corners = 2pt, drop shadow, very
        thick, draw=gray] (0, 0)
        rectangle (8,10);
        \draw (4, 11) node{\scriptsize \textbf{Host A}};
        % vm for host 1
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (0, 0)
        rectangle (8,3);
        \draw (4, 1.5) node{\scriptsize \color{White}{\textbf{VM 1}}};        
        % host 2
        \draw[fill=blue!5, rounded corners = 2pt, drop shadow, very
        thick, draw=gray] (10, 0)
        rectangle (18,10);
        \draw (14, 11) node{\scriptsize \textbf{Host B}};
        % vm for host 1
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (10, 0)
        rectangle (18,4);
        \draw (14, 2) node{\scriptsize \color{White}{\textbf{VM 2}}};        
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (10, 4)
        rectangle (18,6);
        \draw (14, 5) node{\scriptsize \color{White}{\textbf{VM 3}}};        
        % capped capacity
        \path [draw, thick, color=red!80, dashed] (0, 8) -- (8, 8);
        \draw (4, 8.7) node{\scriptsize \color{Black!60}{\textbf{CC}}};
        \path [draw, thick, color=red!80, dashed] (10, 8) -- (18, 8);
        \draw (14, 8.7) node{\scriptsize \color{Black!60}{\textbf{CC}}};
      \end{tikzpicture} \quad\quad\quad
    \centering
    \begin{tikzpicture}[y=.25cm, x=.25cm,font=\sffamily, scale=0.7]
        % host 1
        \draw[fill=blue!5, rounded corners = 2pt, drop shadow, very
        thick, draw=gray] (0, 0)
        rectangle (8,10);
        \draw (4, 11) node{\scriptsize \textbf{Host A}};
        % vm for host 1
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (0, 0)
        rectangle (8,3);
        \draw (4, 1.5) node{\scriptsize \color{White}{\textbf{VM 1}}};        
        % host 2
        \draw[fill=blue!5, rounded corners = 2pt, drop shadow, very
        thick, draw=gray] (10, 0)
        rectangle (18,10);
        \draw (14, 11) node{\scriptsize \textbf{Host B}};
        % vm for host 1
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (10, 0)
        rectangle (18,4);
        \draw (14, 2) node{\scriptsize \color{White}{\textbf{VM 2}}};        
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (10, 4)
        rectangle (18,6);
        \draw (14, 5) node{\scriptsize \color{White}{\textbf{VM 3}}};        
        % capped capacity
        \path [draw, thick, color=red!80, dashed] (0, 6) -- (8, 6);
        \draw (4, 6.7) node{\scriptsize \color{Black!60}{\textbf{CC}}};
      \end{tikzpicture}
    \label{fig:lb}
  } \\
\centering
  \subfloat[{\small Improves~robustness~after~powering
  off a host}]{
    \centering
    \begin{tikzpicture}[y=.25cm, x=.25cm,font=\sffamily, scale=0.7]
        % host 1
        \draw[fill=blue!5, rounded corners = 2pt, drop shadow, very
        thick, draw=gray] (0, 0)
        rectangle (8,10);
        \draw (4, 11) node{\scriptsize \textbf{Host A}};
        % vm for host 1
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (0, 0)
        rectangle (8,3);
        \draw (4, 1.5) node{\scriptsize \color{White}{\textbf{VM 1}}};        
        % host 2
        \draw[fill=blue!5, rounded corners = 2pt, drop shadow, very
        thick, draw=gray] (10, 0)
        rectangle (18,10);
        \draw (14, 11) node{\scriptsize \textbf{Host B}};
        % vm for host 1
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (10, 0)
        rectangle (18,3);
        \draw (14, 1.5) node{\scriptsize \color{White}{\textbf{VM 2}}};        
        % capped capacity
        \path [draw, thick, color=red!80, dashed] (0, 8) -- (8, 8);
        \draw (4, 8.7) node{\scriptsize \color{Black!60}{\textbf{CC}}};
        \path [draw, thick, color=red!80, dashed] (10, 8) -- (18, 8);
        \draw (14, 8.7) node{\scriptsize \color{Black!60}{\textbf{CC}}};
      \end{tikzpicture} \quad\quad\quad
      \begin{tikzpicture}[y=.25cm, x=.25cm,font=\sffamily, scale=0.7]
        % host 1
        \draw[fill=blue!5, rounded corners = 2pt, drop shadow, very
        thick, draw=gray] (0, 0)
        rectangle (8,10);
        \draw (4, 11) node{\scriptsize \textbf{Host A}};
        % vm for host 1
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (0, 0)
        rectangle (8,3);
        \draw (4, 1.5) node{\scriptsize \color{White}{\textbf{VM 1}}};        
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (0, 3)
        rectangle (8,6);
        \draw (4, 4.5) node{\scriptsize \color{White}{\textbf{VM 2}}};        
        % host 2
        \draw[fill=blue!5, rounded corners = 2pt, drop shadow, very
        thick, draw=gray, dashed] (10, 0)
        rectangle (18,10);
        \draw (14, 11) node{\scriptsize \textbf{Host B}};
        \draw (14, 5) node{\scriptsize \color{Black!80}{\textbf{Stand-by}}};
        % capped capacity
        % \path [draw, thick, color=red!80, dashed] (0, 6) -- (8, 6);
        % \draw (4, 6.7) node{\scriptsize \color{Black!60}{\textbf{CC}}};
      \end{tikzpicture}
    \label{fig:poweroff}
}
 \\
 \centering
  \subfloat[{\small Balance robustness after
  powering on a host}]{
    \centering
    \begin{tikzpicture}[y=.25cm, x=.25cm,font=\sffamily, scale=0.7]
        % host 1
        \draw[fill=blue!5, rounded corners = 2pt, drop shadow, very
        thick, draw=gray] (0, 0)
        rectangle (8,10);
        \draw (4, 11) node{\scriptsize \textbf{Host A}};
        % vm for host 1
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (0, 0)
        rectangle (8,4);
        \draw (4, 2) node{\scriptsize \color{White}{\textbf{VM 1}}};        
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (0, 4)
        rectangle (8,8);
        \draw (4, 6) node{\scriptsize \color{White}{\textbf{VM 2}}};        
        % host 2
        \draw[fill=blue!5, rounded corners = 2pt, drop shadow, very
        thick, draw=gray, dashed] (10, 0)
        rectangle (18,10);
        \draw (14, 11) node{\scriptsize \textbf{Host B}};
        \draw (14, 5) node{\scriptsize \color{Black!80}{\textbf{Stand-by}}};
        % capped capacity
        % \path [draw, thick, color=red!80, dashed] (0, 6) -- (8, 6);
        % \draw (4, 6.7) node{\scriptsize \color{Black!60}{\textbf{CC}}};
      \end{tikzpicture} \quad\quad\quad
    \begin{tikzpicture}[y=.25cm, x=.25cm,font=\sffamily, scale=0.7]
        % host 1
        \draw[fill=blue!5, rounded corners = 2pt, drop shadow, very
        thick, draw=gray] (0, 0)
        rectangle (8,10);
        \draw (4, 11) node{\scriptsize \textbf{Host A}};
        % vm for host 1
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (0, 0)
        rectangle (8,4);
        \draw (4, 2) node{\scriptsize \color{White}{\textbf{VM 1}}};        
        % host 2
        \draw[fill=blue!5, rounded corners = 2pt, drop shadow, very
        thick, draw=gray] (10, 0)
        rectangle (18,10);
        \draw (14, 11) node{\scriptsize \textbf{Host B}};
        % vm for host 1
        \draw[fill=BrickRed!50, rounded corners=2pt, thick, draw=gray] (10, 0)
        rectangle (18,4);
        \draw (14, 2) node{\scriptsize \color{White}{\textbf{VM 1}}};        
        % capped capacity
        \path [draw, thick, color=red!80, dashed] (0, 8) -- (8, 8);
        \draw (4, 8.7) node{\scriptsize \color{Black!60}{\textbf{CC}}};
        \path [draw, thick, color=red!80, dashed] (10, 8) -- (18, 8);
        \draw (14, 8.7) node{\scriptsize \color{Black!60}{\textbf{CC}}};
      \end{tikzpicture}
    \label{fig:poweron}
 }
  \caption{Power cap distribution scenarios. Left-hand figures
    correspond to hosts status before distribution;
    right-hand figures show hosts status after. Power-capped capacity
    is not shown when the power cap of the host equals its peak
    power. (CC: Power-capped capacity)}
 \end{figure}


==> util-macros.tex <==
% -*- TeX-master: "paper.tex"; TeX-PDF-mode: t -*-

% some useful macros

% Tuple typesetting
% Adds triangle brackets and spaces commas.  ie $\tup{1,2,3}$
% Arguments can be enclosed in braces or angle brackets
\makeatletter
\def\tup{%
  \def\tupInside\tupStart##1,##2\tupEnd{%
    ##1
    \def\tempa{}\def\tempb{##2}
    \ifx\tempa\tempb\else
    ,\;\tupInside\tupStart##2\tupEnd
    \fi}
  \def\tupBraces##1{\left\langle\tupInside\tupStart##1,\tupEnd\right\rangle}
  \def\tupBrackets<##1>{\tupBraces{##1}}
  \@ifnextchar<\tupBrackets\tupBraces}
\makeatother

\definecolor{xxxcolor}{rgb}{0.8,0,0}
\makeatletter
\long\def\XXX{\@ifnextchar[{\@XXX}{\@XXX[]}}
\long\def\@XXX[#1]{\@ifnextchar[{\@@@XXX{#1}}{\@@XXX{#1}}}
\ifnotes
% Show XXX comments
\long\def\@@XXX#1{{\color{xxxcolor} $<$XXX #1$>$\xspace}}
\long\def\@@@XXX#1[#2]{{\color{xxxcolor} $<$XXX (#1) #2$>$\xspace}}
\else
% Hide XXX comments
\long\def\@@XXX#1{\ignorespaces}
\long\def\@@@XXX#1[#2]{\ignorespaces}
\fi
\makeatother

\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishlisttwo}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{2em} \setlength{\labelwidth}{1.5em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
    \end{list}  }


% time macros
\newcount\hour
\newcount\minute
\hour=\time
\divide \hour by 60
\minute=\time
\loop \ifnum \minute > 59 \advance \minute by -60 \repeat
\def\now{%
\ifnum \hour<13
\ifnum \hour<1 12:\else\number\hour:\fi
\ifnum \minute<10 0\fi                 
\number\minute%                      
\ifnum \hour<12 \ am \else \ pm \fi
\else \advance \hour by -12 \number\hour:%
\ifnum \minute<10 0\fi            
\number\minute%                 
\ pm \fi%
}

% common symbols
%   mbox is used to allow macro to be used 
%   in both text and math modes
\newcommand{\latency}{\mbox{$L$}\xspace}
\newcommand{\thruput}{\mbox{$T$}\xspace}
\newcommand{\throughput}{\thruput\xspace}
\newcommand{\oio}{\mbox{$Q$}\xspace}
\newcommand{\iops}{\mbox{$IOPS$}\xspace}
\newcommand{\slope}{\mbox{$m$}\xspace}
\newcommand{\intercept}{\mbox{$C$}\xspace}
\newcommand{\hitrate}{\mbox{$h$}\xspace}

\newcommand{\lqslope}{LQ-slope\xspace}
\newcommand{\lqplot}{LQ-plot\xspace}

% common symbols, with specified subscript

\newcommand{\latencysub}[1]{\mbox{$L_{#1}$}\xspace}
\newcommand{\thruputsub}[1]{\mbox{$T_{#1}$}\xspace}
\newcommand{\oiosub}[1]{\mbox{$Q_{#1}$}\xspace}
\newcommand{\slopesub}[1]{\mbox{$m_{#1}$}\xspace}

% XXX not sure which looks better 
% \newcommand{\timesub}[1]{\mbox{$t_{#1}$}\xspace}
\newcommand{\timesub}[1]{\mbox{$\tau_{#1}$}\xspace}

